A Flexible Framework for Designing Trainable Priors with Adaptive Smoothing and Game Encoding

We introduce a general framework for designing and training neural network layers whose forward passes can be interpreted as solving non-smooth convex optimization problems, and whose architectures are derived from an optimization algorithm. We focus on convex games, solved by local agents represented by the nodes of a graph and interacting through regularization functions. This approach is appealing for solving imaging problems, as it allows the use of classical image priors within deep models that are trainable end to end. The priors used in this presentation include variants of total variation, Laplacian regularization, bilateral filtering, sparse coding on learned dictionaries, and non-local self similarities. Our models are fully interpretable as well as parameter and data efficient. Our experiments demonstrate their effectiveness on a large diversity of tasks ranging from image denoising and compressed sensing for fMRI to dense stereo matching.

==> A Flexible Framework for Designing Trainable Priors with Adaptive Smoothing and Game Encoding/abstract.tex <==
% We introduce a general framework for designing and learning neural
% networks whose forward passes can be interpreted as solving convex optimization
% problems, and whose architectures are derived from an optimization algorithm.
% We focus on 
% non-cooperative convex games, solved by local agents represented by the nodes of a graph and interacting
% through regularization functions. This approach is appealing for
% solving imaging problems, as it allows the use of
% classical image priors within deep models that are trainable end to end. The
% priors used in this presentation include variants of total variation, Laplacian regularization, bilateral filtering, sparse
% coding on learned dictionaries, and non-local self similarities. 
% Our models are parameter efficient and fully interpretable, and our experiments
% demonstrate their effectiveness on a large diversity of tasks ranging from image denoising and
% compressed sensing for fMRI to dense stereo matching.

We introduce a general framework for designing and training neural network layers whose forward passes can be interpreted as solving non-smooth convex optimization problems, and whose architectures are derived from an optimization algorithm.
We focus on convex games, solved by local agents represented by the nodes of a graph and interacting
through regularization functions. This approach is appealing for solving imaging problems, as it allows the use of
classical image priors within deep models that are trainable end to end. The
priors used in this presentation include variants of total variation, Laplacian regularization, bilateral filtering, sparse
coding on learned dictionaries, and non-local self similarities. 
Our models are fully interpretable as well as parameter and data efficient. Our experiments
demonstrate their effectiveness on a large diversity of tasks ranging from image denoising and
compressed sensing for fMRI to dense stereo matching.
 
% In this context, we adopt a more general and flexible point of view than the standard convex opti-
% mization paradigm, and consider formulations to represent data based on non-cooperative games

==> A Flexible Framework for Designing Trainable Priors with Adaptive Smoothing and Game Encoding/background.tex <==
\paragraph{Classical image priors.}
Inverse imaging problems are often solved by minimizing a data fitting term with
respect to model parameters, regularized with a penalty that encourages
solutions with a particular structure. 
In image processing, the community long focused on designing handcrafted 
priors such as sparse coding on learned dictionaries
\cite{elad2006image,mairal2014sparse}, diffusion operators \cite{perona1990}, total variation~\cite{rudin1992nonlinear}, and
% non-local self similarities \cite{buades2005non, dong2012nonlocally}, which is 
non-local self similarities \cite{buades2005non}, which is 
a key ingredient of successful restoration algorithms such as BM3D \cite{dabov2009bm3d}. 
However these methods are now often outperformed by deep
learning models \cite{liu2018non,zhang2017beyond,zhang2018ffdnet},
which leverage pairs of corrupted/clean training images in a supervised fashion.

\vs
\paragraph{Bilevel optimization.}
%\textit{only for sparse coding  B : not only sparse coding. Nubmer of unrolled architectures is countless ; we do much more; a general framework was missing.}
%In order to embed domain priors in learning algorithms, a common approach is to solve a \textit{bi-level optimization problem},
A simple method for mixing data representation learning with optimization is to use a bi-level formulation~\cite{mairal2011task}. 
% A classical way to use a data representation obtained by an optimization-based model into a supervised learning problem is 
% to design a bi-level formulation~\cite{mairal2011task}. 
For instance, assuming that one is given pairs $(\xb_i,\yb_i)_{i=1\dots n}$ of corrupted/clean signals with $\xb_i$ and $\yb_i$ in $\Real^m$, 
one may consider the following bi-level objective
%where an optimization problem regularized with a certain prior is included as a constraint in a learning problem. Mathematically, this can be formulated as a stochastic optimization problem with an equality constraint:
\begin{equation} \label{eq:bilevel}
   \min_{\thetab \in {\Theta}, \Wb \in \Real^{m \times p}}  
   \frac{1}{n}\sum_{i=1}^n L( \yb_i, \Wb \alphab^\star_{\thetab}( \xb_i) ) 
     ~~~~\text{where}~~~~ \alphab^\star_{\thetab}(\xb_i) \in \argmin_{\alphab \in \Real^p} h_{\thetab}(\xb_i,\alphab), 
  % \left [ f_S(\hat{x}_S^*(\theta) , \theta) \right ] \quad
  %  \text{s.t.} \quad  \hat{x}_S^*(\theta) \approx \argmin_{x} h_S(x,\theta) ,
  % why linear WZ ? looks very specific
\end{equation}
where $\thetab$ is a set of model parameters, $\Wb\alphab^\star_{\thetab}(\xb_i)$ is a prediction which is compared to $\yb_i$ through
 a loss function $L:\mathbb{R}^m\times \mathbb{R}^m \rightarrow \mathbb{R}^+$,
and the data representation $\alphab_{\thetab}^\star(\xb_i)$ in $\Real^p$ is obtained by minimizing some function $h_{\thetab}$.
%B : why h_theta ? can be misleading 
Note that for simplicity, we have considered here a multivariate regression problem, where given a signal $\xb$ in $\Real^m$, we want to predict 
another signal $\yb$ in $\Real^m$, but this formulation also applies to classification problems.
It was first introduced for sparse coding in~\cite{mairal2011task,yang2012coupled} and it has recently been extended to the case 
when~$\alphab^\star_{\thetab}(\xb_i)$ is 
replaced by an approximate minimizer of $h_{\thetab}$.
% where $f_S$ is the sampled upper level objective, $g_S$ is the sampled lower objective corresponding to a regularized optimisation problem introduced before and
% $S$ is a random variable and $\hat{x}_S^*(\theta)$ is the returned value of an algorithm that approximately finds a local minimum of $hs$.
% Solving the bi-level optimization problem is difficult due to the complicated relations of the upper-level problem on $\theta$ induced by $x^*(\theta)$.
% Furthermore we only have access to $\hat{x}^*$ which is the approximate solution returned by an iterative algorithms
%  that finds a local minimum of $h$.
%A commonly used approach is to assume that $\hat{x}^* = x^*$ and compute $\nabla_{\theta} x^*$ by implicit differentiation \cite{mairal2011task} leveraging optimality conditions of the lower problems.
% Nowadays unrolling based approaches are gaining more and more popularity \cite{shaban2018truncated}. 
% The general idea is to unroll iterations of the inference algorithms
% which yields an approximated solution $\hat{x}^*$, see it as a computational graph and compute $\nabla_{\theta} x^*$
  % by automatic differentiation \cite{gregor2010learning}.
% % That inference can be inserted in various deep learning architectures. 
% % More The main idea is to treat the iterative optimization algorithm in the lower problem as a dynamical system . 
% This approach presents several advantages : unlike implicit differentiation this is not sensitive to the optimality of $\hat{x^*}$
% hyperaprameters which control the lower optimisation process  can also be learnt \cite{liu2018alista,gregor2010learning}. In this paper we refer to this general concept as
% as \textit{optimization-driven} networks.
% In fact, it can be conveineint to consider this unrolled algorithm as neural network.
\vsp
\paragraph{Unrolled algorithms.}
% A common approach to solving (\ref{eq:bilevel}) consists in choosing an iterative method for minimizing $h_{\thetab}$, defining~$\alphab^\star_{\thetab}(\xb_i)$ as the output of the optimization method after $K$ iterations,
% and then see the sequence of operations performed by the optimization method as a computational graph and compute 
% $\nabla_{\thetab} \zb_{\thetab}^\star$ by automatic differentiation.
A common approach to solving (\ref{eq:bilevel}) consists in choosing an iterative method for minimizing $h_{\thetab}$ and then define ~$\alphab^\star_{\thetab}(\xb_i)$ as the output of the optimization method after $K$ iterations. The sequence of operations performed by the optimization method can be seen as a computational graph and $\nabla_{\thetab} \zb_{\thetab}^\star$ can be computed by automatic differentiation.
This often yields neural-network-like computational graphs, which we call \emph{optimization-driven layers}.
Such architectures have found multiple applications such as training of conditional random fields \cite{zheng2015conditional},
stabilization of generative adversarial networks \cite{metz2016unrolled}, structured prediction \cite{belanger2017end}, or hyper-parameters tuning \cite{maclaurin2015gradient}.
For image restoration, various optimization problems have been explored including for example sparse coding \cite{lecouat2020fully,simon2019rethinking,zhang2018ista}, non linear diffusion
\cite{chen2016trainable} and differential operator regularization \cite{lefkimmiatis2018universal}.
Many inference algorithms have been investigated 
including proximal gradient descent \cite{lefkimmiatis2018universal, simon2019rethinking}, 
ADMM \cite{fletcher2018plug}, half quadratic spliting \cite{zoran2011learning}, or augmented Lagrangian~\cite{romano2017little}.
 

%\textit{B cite cvx layers (differentiable convex optim layers) \cite{cvxpylayers2019}}
%Eventually brieffly mention sparsity and group sparsity for networks compression, to avoid any amibguties (we seek sparsity for the activations whereas these methods try to achieve
%sparse parameters for the neural net).

 
%\cite{djolonga2017differentiable} submodular problems
% CRF unrolled 
% 
% \paragraph{Smoothing techniques}
% 
% Given a convex function $f$, we introduce the Moreau envelope $F_\kappa$, defined as the infimal convolution
% \begin{equation}
%     F_\kappa(x) = \min_{y \in \mathbb{R} } f(y) + \frac{\kappa}{2} \left \| y- x \right \|^2.
% \end{equation}
% 
% It turns out that we have the following properties:
% \begin{itemize}
%     \item $f$ and $F_\kappa$ have the same minimum and same minimizers.
%     \item $F_\kappa$ is differentiable and its graident is $\kappa$-Lipschitz
%     \item $\nabla F_\kappa = \kappa (x-p_\kappa(x))$, where $p_\kappa(x)$
% \end{itemize}
% 
% Consider now the Moreau-Yosida regularization $\Psi_\kappa$ of a non-smooth convex function $\psi$. Then, we may consider the optimization problem: 
% \begin{equation}
%     \min_{x \in \mathbb{R}^n} f(x) + \Psi_\kappa(x),
% \end{equation}
% instead of $\min_{x \in \mathbb{R}^n} f(x)+\psi(x) $. However, both problems do not admit the same
% solutions, and if $\psi$ is sparsity-inducing, it may not be the case for $\Psi_\kappa$ .
% 
% \paragraph{Game Theory for distributed optimization } 
% Game theory is oftens used to model selfish behaviors in distributed systems. We will focus on non-cooperative game model with finite number of players.
% Given a set of n players, we express the parameters of the game as $\xb=(\xb_1,\xb_2,\cdots,\xb_n)$.
% Each player $i$ has a loss function $\ell_i(\xb_i, \xb_{-i}) \in \mathbb{R}$. The player seeks to achieve the minimum value of $\ell_i$ but is only able to control $\xb_i$.\footnote{
% We write $\xb = (\xb_i, \xb_{-i})$ , where  $\xb_{-i}$  refers to all the parameters different from $\xb_i$ .}
% 
% A {pure Nash equilibrium} is a vector $\xb^*$ such that for all $i$ and all $\tilde{\xb}_i \in X_i$,
% 
% \begin{equation}
%     \ell_i(\xb_i^*,\xb_{-i}^*) \leq \ell_i(\tilde{\xb}_i,\xb_{-i}^*).
% \end{equation}
% 
% 
% We can also define {simulatenous gradient} $  F(\xb)=[ \nabla_{1} \ell_1(\xb), \nabla_{2} \ell_2(\xb), \cdots, \nabla_{n} \ell_n(\xb) ]^\top,$ and {simultaneous gradient descent} with stepsize $\gamma$
% \begin{equation}
%      \xb_{t+1} = \xb_t-\gamma F(\xb_t).
% \end{equation}
% To the best of our knowledge there is no general result about convergence of simultaneous gradient descent in the general case. 


==> A Flexible Framework for Designing Trainable Priors with Adaptive Smoothing and Game Encoding/ccl.tex <==
\vsp
We have presented a general framework based on non-cooperative games to train
end-to-end imaging priors. Our experiments demonstrate the flexibility and the effectiveness
of our approach  on diverse tasks ranging from image denoising to fMRI reconstruction and dense stereo matching.
%
% We believe that the performance of such approaches is encouraging given the small model sizes
% and the conceptual simplicity of the studied priors. In the future, we will experiment
% on other modalities such as 3D point clouds and meshes, which should naturally benefit from the sparsity-inducing graph regularization functions introduced in our paper.
Beyond image processing, we believe that the issue of interpretability is important.
We consider models with a clear mathematical description of the
decision function they produce. As a by-product, our models are also more
parameter efficient than classical deep learning models. We believe that these
are important steps to build systems that should not be seen as
black boxes anymore, that produce explanable decisions, and that do not require
training a system for days on a huge corpus of annotated data. These are
important questions, which we are planning to address
explicitly in the~future.


==> A Flexible Framework for Designing Trainable Priors with Adaptive Smoothing and Game Encoding/experiments.tex <==
We consider three different tasks, illustrated with various combinations of regularization functions
in order to demonstrate the wide applicability of our approach and its flexibility.
A software package and additional details are provided in the supplementary material for reproducibility purposes.

\begin{table}[htb]
    % \vspace{-0.4cm}
    \centering
    \caption{\textbf{Grayscale denoising} on BSD68, training on BSD400 for all methods.
        Performance in terms of average PSNR. Tiny CNN is a CNN baseline with few parameters. See Appendix~\ref{app:quant} for qualitative results.}\label{tab:denoising}
    \label{gray_table}
    {
        \small
        \begin{tabular}{@{}lcccccc@{}}
            \toprule
            \multirow{2}{*}{Method}                                  & \multirow{2}{*}{Params $ \quad\quad$} & \multicolumn{4}{c}{Noise Level ($\sigma$)}                                                             \\
                                                                     &                         & 5                                          & 15                & 25                & 50                \\
            \midrule
                        Tiny CNN   \textit{(ours)}                                        & 326                     & 35.17                                      & 29.42             & 26.90             & 24.06             \\
            Tiny CNN   \textit{(ours) }                                       & 1200                    & 36.47                                      & 30.36             & 27.70             & 24.60             \\


            BM3D \cite{dabov2007image}                               & -                       & 37.57                                      & 31.07             & 28.57             & 25.62             \\
            LSCC \cite{mairal2009non}                                & -                       & 37.70                                      & 31.28             & 28.71             & 25.72             \\
            % \midrule
            CSCnet \cite{simon2019rethinking}                        & 62k                     & 37.69                                      & 31.40             & { 28.93}          & 26.04             \\
            {GroupSC} \cite{lecouat2020fully}                        & {68k}                   & {37.95}                                    & 31.71             & 29.20             & 26.17             \\
            FFDNet \cite{zhang2018ffdnet}                            & 486k                    & N/A                                        & 31.63             & 29.19             & 26.29             \\
            DnCNN   \cite{zhang2017beyond}                           & 556k                    & {37.68}                                    & {31.73}           & 29.22             & 26.23             \\
            NLRN  \cite{liu2018non}                                  & 330k                    & {37.92}                                    & \textbf{31.88}    & \textbf{29.41}    & \textbf{26.47}    \\
            % \midrule

            \midrule
            \midrule
            \multicolumn{6}{l}{\textit{Pixel-reconstruction}}                                                                                                                                                    \\
            {TV}  \textit{symmetric}                                 & 288                      & 36.91                                      & 30.27             & 27.66             & 24.51             \\
            % {TV} \textit{symmetric}   - \textit{extra-grad}                                         & 144                     & 37.02                                      & 30.33              & 27.82               & 24.81              \\
            % {TV}  \textit{assymetric}                                                              & 240                     & 36.83                                      & 30.49              & 27.99               & 24.93              \\
            {TV}   \textit{assymetric}   - \textit{extra-grad}       & 480                     & 37.30                                      & 30.76             & 28.24             & 25.32             \\
            % \midrule
            {Laplacian}  \textit{symmetric}                          & 288                      & 35.17                                      & 28.42             & 26.14             & 23.70             \\
            % {Laplacian} \textit{symmetric}    - \textit{extra-grad}                                 & 144                     & 33.87                                      & 28.14              & 25.91               & 23.45              \\
            % {Laplacian}   \textit{assymetric}                                                       & 240                     & 35.20                                      & 28.48              & 26.17               & 23.78              \\
            {Laplacian}  \textit{assymetric}   - \textit{extra-grad} & 480                     & 35.20                                      & 28.46             & 26.39             & 23.77             \\
            % \midrule
            % {Non-local TV} \textit{assymmetric}                                                     & 154                     & 37.25                                      & 30.86              & 28.28               & 25.42              \\
            % {Non-local TV} \textit{assymmetric}   (several $\kappa$)                                & 235                     & 37.12                                      & { 31.01 }          & 28.37               & 25.24              \\
            % {Non-local TV} \textit{assymmetric}  -   \textit{extra-grad}                            & 226                     & \textbf{37.83}                             & 30.98              & 28.34               & 25.31              \\
            

            {Bilateral}  -   \textit{extra-grad}                     & 146                     &                                             36.75&29.89&27.20&23.72                                                           \\

            {Bilateral TV}  -   \textit{extra-grad}                  & 146                     &                                   36.94 & 30.46 & 27.78 & 24.52                                                          \\

                       
            
            {Non-local TV}  -   \textit{extra-grad}                  & 307                     & 37.53                                      & 31.03             & 28.50             & 25.26             \\
            % \midrule
            % {Non-local Laplacian} \textit{assymmetric}                                              & 154                     & 37.31                                      & 30.75              & 28.33               & 25.15              \\
            % {Non-local Laplacian} \textit{assymmetric}   (several $\kappa$)                         & 235                     & 37.53                                      & {31.01 }           & 28.37               & \underline{ 25.47} \\
            % {Non-local Laplacian} \textit{assymmetric}  -   \textit{extra-grad}                     & 226                     & 37.51                                      & 30.99              & 28.34               & 25.13              \\
            {Non-local Laplacian}  -   \textit{extra-grad}           & 307                     & 37.54                                      & 31.00             & 28.47             & 25.46             \\
 \midrule
            \midrule
            \multicolumn{6}{l}{\textit{Patch-reconstruction}}                                                                                                                                                    \\

            Sparse Coding (SC)                                           & {68k}                   & 37.84                                      & 31.46             & 28.90             & 25.84             \\
            % Sparse Coding + {Barzilai-Borwein}                                       & {68k}                   & 37.85                                      & 31.46             & 28.91               & 25.84             \\
            Sparse Coding + {Variance}                               & {68k}                   & 37.83                                      & 31.49             & 29.00             & 26.08             \\
            Sparse Coding + {TV}                                     & {68k}                   & 37.84                                      & 31.50             & 29.02             & 26.10             \\
            Sparse Coding + {TV}   + {Variance} $\quad \quad$        & {68k}                   & 37.84                                      & 31.51             & 29.03             & 26.09             \\
            % Sparse Coding + {TV}   + {Variance}  + {Barzilai-Borwein}                 & {68k}                   & 37.86                                      & 31.52             & 29.04               & 26.04             \\
            % \midrule
            % {{Non-local group} - \textit{symmetric} }                         & {68k}                   & 37.94                                      & 31.67             & 29.17               & 26.16             \\
            {{Non-local group}    }                                  & {68k}                   & 37.95                                      & 31.69             & 29.19             & 26.19             \\
            % {{Non-local group} - \textit{assymetric}   }         + {TV}       & {68k}                   & 37.96                                      & 31.71             & 29.22               & 26.26             \\
            {{Non-local group}     + {Variance}}                     & {68k}                   & \textbf{37.96}                             & 31.70             & 29.22             & 26.28             \\
            % {{Non-local group} -  \textit{assymetric}   + {Variance}}  + {TV} & {68k}                   & 37.95                                      & 31.71             & \underline{29.24  } & 26.30             \\
            {GroupSC + {Variance}}                                   & {68k}                   & \textbf{37.96}                             & \underline{31.75} & \underline{29.24} & \underline{26.34} \\


            \bottomrule
        \end{tabular}
    }
    \vspace{-0.2cm}
\end{table}

\vs
\paragraph{Image denoising.}
For image denoising experiments, we use the
standard setting of \cite{zhang2017beyond} with BSD400 \cite{martin2001database}
as a training set and on BSD68 as a test set.
% For patch based models we choose a patch size of $9\times9$ and dictionary with 256 atoms for our models. For the training, we randomly
% extract patches of size $56\times56$; whereas we train pixel level models on the full size images.
We optimize the parameters of our models using Adam~\cite{kingma2014adam}
and also use the backtracking strategy described in Section~\ref{sec:tricks} that automatically
decreases the learning rate by a factor 0.5 when the training loss diverges.
For the non-local models, we follow~\cite{lecouat2020fully} and update the similarity matrices three times during the inference step.
We use the parametrization with the $\Cb$ matrix for our patch-based experiments.
% 
We also combine our variance regularization with~\cite{lecouat2020fully}.
%
Additional training details and hyperparameters choices can be found in Appendix \ref{appendix:training}.
We report performance in terms of averaged PSNR in Table \ref{tab:denoising}, and
more detailed tables with additional results are available in Appendix~\ref{app:quant} for pixel-level models,
and for the patch-based models involving a dictionary~$\Db$.
% \begin{center}
%     [B : qualitative results for denoising here on in appendix ?]
% \end{center}
% \begin{center}
%     [B : Table inference time TV / NLTV ]
% \end{center}
Our models based on non-local sparse approximations perform better than the competing deep learning models with the exception
of \cite{liu2018non} for $\sigma \geq15$ with much fewer parameters.
In addition, we also observed that our assymetric TV models are almost on par with BM3D
while being significantly faster (see Appendix~\ref{app:quant} for more details) with only a very small amount of parameters.


\vs
\paragraph{Compressed Sensing for fMRI.}
Compressed Sensing for functional magnetic resonance
imaging (fMRI) aims at reconstructing functional MR images from a small number of samples in the Fourier space.
% and accelerating the data acquisition in MRI.
The corresponding inverse problem is
\begin{equation}
    \min_{\yb \in \mathbb{R}^n} \|\Ab \yb - \xb \|^2_2 + \lambda \Psi(\yb),
\end{equation}
where the degradation matrix is $\Ab = \Pb \mathcal{F}$, $\Pb$ is a diagonal binary sampling matrix for a given sub-sampling pattern,
$\mathcal{F}$ is the discrete Fourier transform such that
the observed corrupted signal $\xb$ is in the Fourier domain, and $\Psi$ is a regularization function.
This problem  highlights  the ability of our framework to handle both localized and non
localized constraints.
% , since the data fitting term involves the whole image since the information in
% the fourier space is not spatially localized.
% \vs
% \paragraph{Examples of models for fMRI} :
In our paper, we implemented two models revisiting some well studied priors for compressed sensing in an end-to-end fashion:
\begin{itemize}[leftmargin=*,nosep]
    \item \emph{Pixel reconstruction} with total variation: we aim at solving the optimization for each node
          $\min_{\yb_i \in \mathbb{R} } \left \|  \Ab \yb - \xb  \right \|_2^2 + \text{TV}_i( \yb) $. In the past,
          total variation has been widely used for MRI \cite{lustig2007sparse}, often in combination with sparse regularization in the wavelet domain.
          %   However and to the best of our knowledge, task driven TV has never been studied in previous works.

    \item \emph{Patch encoding on a dictionary with sparse coding}: we solve a collection of optimization problems of the form
          $\min_{\zb_i \in \mathbb{R}^{n} } \left \|  \Ab \hat{\yb}(\zb) - \xb  \ \right \|_2^2 +
              \lambda \|\zb_i\|_1$, with $ {\yb} = \frac{1}{n} \sum_j \Rb_j^\top \Db \zb_j $ the average of the overlapping patches.
          %   Classic fMRI model leverage sparse regularization in some transform domains. 
          Some previous methods have explored dictionary-based reconstruction \cite{ravishankar2010mr},
          but they were not investigated from a task-driven manner with end-to-end training.
          %    \cite{ravishankar2010mr} check that we are not doing the same thing that this paper.
\end{itemize}

In our experiments, we use the same setting as \cite{sun2016deep} for fair comparison:
% We compare our method with recent state of the art methods in the same setting. 
we train and test our models on the brain MRI dataset
% \footnote{Dataset available at \url{https://masi.vuse.vanderbilt.edu/workshop2013/index.php/Segmentation_Challenge_Details}}
studied in that paper.
% The resolution of the images is 256 x 256. 
Our models are trained separately for each sampling rate.
We used the pseudo radial sampling for the matrix $\Pb$ similarly to the other methods.
The reconstruction accuracy are reported in term of PSNR over the test set in Table~\ref{tab:mri}.
%
Our trainable model relying on a trainable TV prior performs surprisingly well given the conceptual simplicity of the prior.
% At the exception og BM3D-MRI, 
% it outperforms the non learning based methods by a large margin. 
Also importantly, it runs significantly faster than all competing methods with
a very small number of parameters.
Furthermore, our trainable sparse coding method for fMRI gives strong performance and exceeds the state of the art for sampling rates larger than 30\%.
Note that architecture choices (patch and dictionary size) of our models are the same as for the denoising task, and we did not try to optimize them for the considered task,
thus demonstrating the robustness of our approach.

\begin{table}[]
    \small
    \centering
    \caption{\textbf{Compressed sensing for fMRI} on the MR brain dataset  using a pseudo radial sampling pattern. Performance  comparisons in terms of PSNR (dB).
    }\label{tab:mri}
    \begin{tabular}{lcccccl}
        \toprule
        Method                                 & Params & 20 \%              & 30 \%              & 40\%                & 50\%               & Test time     \\
        \midrule
        % Zero-filling                              & 29.96              & 32.59              & 34.76               & 36.73              & -      & 0.0013s       \\
        TV   \cite{lustig2007sparse}           & -      & 35.20              & 37.99              & 40.00               & 41.69              & 0.731s (cpu)  \\
        RecPF  \cite{yang2010fast}             & -      & 35.32              & 38.06              & 40.03               & 41.71              & 0.315s (cpu)  \\
        SIDWT                                  & -      & 35.66              & 38.72              & 40.88               & 42.67              & 7.867s (cpu)  \\
        PANO   \cite{qu2014magnetic}           & -      & 36.52              & 39.13              & 40.31               & 41.81              & 35.33s (cpu)  \\
        BM3D-MRI \cite{eksioglu2016decoupled}  & -      & \underline{37.98 } & 40.33              & 41.99               & 43.47              & 40.91s  (cpu) \\
        ADMM-net        \cite{sun2016deep}     & -      & 37.17              & 39.84              & 41.56               & 43.00              & 0.791s (cpu)  \\
        ISTA-net        \cite{zhang2018ista}   & 337k   & \textbf{ 38.73}    & \textbf{40.89}     & {\underline{42.52}} & \underline{44.09 } & 0.143s (gpu)  \\
        \midrule
        {CS-TV} (ours)                         & 140    & 36.80              & 39.63              & 41.58               & 43.46              & 0.015s (gpu)  \\
        % graphNLTV (ours)  &       &       &       &                                 \\
        {CS-Sparse coding} (ours)              & 68k    & 37.80              & 40.50              & 42.46               & {44.16}            & 0.213s (gpu)  \\
        {CS-Sparse coding} + {Variance} (ours) & 68k    & 37.79              & \underline{40.67 } & \textbf{42.54 }     & \textbf{44.17}     & 0.213s (gpu)  \\

        \bottomrule

    \end{tabular}
    \vspace{-0.6cm}

\end{table}

\begin{minipage}[]{.55\textwidth}
    \small
    \captionof{table}[t]{\textbf{Denoising with less data}. Results in terms of average PSNR(dB) on BSD68 with $\sigma=15$. All the models are trained on a similar subset of BSD400 for fair comparaison.}\label{tab:lessdata}

    \begin{tabular}{lrcccc}
        \toprule
        \multirow{2}{*}{Method}      & \multirow{2}{*}{\begin{scriptsize} Params \end{scriptsize}} & \multicolumn{4}{c}{Training images}                                                     \\
                                     &                                                & 400                                 & 200             & 100            & 50             \\ \midrule
        % BM3D & - &  \multicolumn{4}{c}{31.07} \\
        DnCNN \cite{zhang2017beyond} & 556k                                           & \underline{31.73}                               & \underline{31.65}          & \underline{31.47}          & 31.23          \\ \midrule
        TV \textit{extra-grad}       & 480                                            & 30.75                               & 30.72           & 30.67          & 30.66          \\
        SC+Var               & 68k                                            & 31.49                               & 31.49           & \underline{31.47}          & \underline{31.40}          \\
        GroupSC+Var                  & 68k                                            & \textbf{31.75}                      & \textbf{31.66} & \textbf{31.62} & \textbf{31.54} \\
        \bottomrule
    \end{tabular}
\end{minipage}%
% \footnotetext{    {Code available on github \url{ https://github.com/JiaRenChang/PSMNet.}}}
\hspace{0.5cm}
\begin{minipage}[]{.40\textwidth}
    %\vspace*{-0.2cm}
        % \vspace*{0.25cm}

    \captionof{table}[t]{\textbf{Dense stereo matching} fine-tuning on kitti2015 train set, performance reported on the kitti2015 validation set.}
    \centering \small
    % \vspace*{0.13cm}
    \begin{tabular}{lc}
        \toprule
        Model                                             & 3-px error (\%)          \\ \midrule
        {PSMNet} \cite{chang2018pyramid}           & 2.14    $\pm$ 0.04       \\
        \midrule
        {PSMNet}+{TV} 12            & 2.11  $\pm$ 0.03         \\
        {PSMNet}+{TV} 24            & 2.11   $\pm$  0.04       \\
        {PSMNet}+{TV} \textit{extra} & \textbf{2.10 $\pm$ 0.03} \\
        \bottomrule
    \end{tabular}
    \label{tab:stereo}
    % \end{table}
\end{minipage}
\vspace{0.2cm}

\paragraph{Dense Stereo Matching.}
Our approach can be used to provide a generic regularization module that can easily be integrated into various neural architectures.
We showcase its versatility by using it for deep stereo matching \cite{scharstein2002taxonomy}.
Given aligned image pairs, the goal is to compute disparity $\bf d$ for each pixel.
% solved with various algorithms (graph cuts, simulated annealing)
Traditionally stereo matching is formulated as minimization of an energy function
$ E_{\text{data}}(\db) + \lambda E_{\text{smooth}}(\db)$
where the data term, $E_{\text{data}}$ measures how well $\db$ agrees with the input image
pairs,  $E_{\text{smooth}}$  enforces consistency among neighboring pixels’ disparities: TV is a commonly chosen regularizer.
% $E_{\text{smooth}}$ is a regularization term, TV is commonly chosen prior 
% as it leverages the fact that close pixel are likely to belong to the same objects and then share common disparity values.
Recent deep learning methods tackle the problem as a supervised regression to estimate continuous
disparity map given pairs of stereo views and ground truth disparity maps \cite{chang2018pyramid}.
%
We propose to combine our smoothing TV block with a state-of-the-art deep learning model \cite{chang2018pyramid}.
In practice, we combine our block with a pretrained model
on the SceneFlow \cite{MIFDB16} dataset,  and fine-tune the pretrained model on the  kitti2015 \cite{geiger2012we}
train set, following the training procedure described in \cite{chang2018pyramid}.
%  \noindent\begin{minipage}{.5\textwidth}
%
%
We used
the original implementation of \cite{chang2018pyramid} available online and did not
change any hyperparameters.
We report in Table~\ref{tab:stereo} the performance on the validation set in term of 3 pixels error
which counts predicted pixel as correct if the disparity deviates from the ground truth from 3 pixels or less.
% We report the performance of all the models after 200 epochs of training.
We ran the experiment 10 times for each model (with and without the TV regularization).
We observed that our TV block introduces very few additional parameters and consistently boosts performances.

% \end{minipage}%

% \begin{minipage}[t]{.53\textwidth}
%     We used
%     the original implementation of \cite{chang2018pyramid} available online and did not
%     change any hyperparameters.
%     We report in Table~\ref{tab:stereo} the performance on the validation set in term of 3 pixels error
%     which counts predicted pixel as correct if the disparity deviates from the ground truth from 3 pixels or less.
%     % We report the performance of all the models after 200 epochs of training.
%     We ran the experiment 10 times for each model (with and without the TV regularization).
%     We observed that our TV block introduces very few additional parameters and consistently boosts performances.

% \end{minipage}%
% % \footnotetext{    {Code available on github \url{ https://github.com/JiaRenChang/PSMNet.}}}
% \hspace{0.3cm}
% \begin{minipage}[t]{.40\textwidth}
%     \vspace*{-0.2cm}
%     \captionof{table}[t]{\textbf{Dense stereo matching} fine-tuning on kitti2015 train set, performance reported on the kitti2015 validation set.}
%     \centering \small
%     \vspace*{-0.2cm}
%     \begin{tabular}{lc}
%         \toprule
%         Model                                             & 3-px error (\%)          \\ \midrule
%         \textbf{PSMNet} \cite{chang2018pyramid}           & 2.14    $\pm$ 0.04       \\
%         \midrule
%         \textbf{PSMNet}+\textbf{TV} 12 (ours)             & 2.11  $\pm$ 0.03         \\
%         \textbf{PSMNet}+\textbf{TV} 24 (ours)             & 2.11   $\pm$  0.04       \\
%         \textbf{PSMNet}+\textbf{TV} \textit{extra} (ours) & \textbf{2.10 $\pm$ 0.03} \\
%         \bottomrule
%     \end{tabular}
%     \label{tab:stereo}
%     % \end{table}
% \end{minipage}

\vs
\paragraph{Training with few examples.}
We conducted denoising experiments with less training data and report corresponding results in Table \ref{tab:lessdata}. We use the code released by the authors for
training DnCNN with less data.
Very interestingly the gap between our best model and CNN-based models increases when decreasing the size of the training set. We believe that this is an appealing feature, particularly relevant for applications in medical imaging or microscopy where the amount of training data can be very limited.

% \begin{table}
%     \centering
%     \small
%     \caption{\textbf{Denoising with a smaller training set }($\sigma=15$). Results in terms of average PSNR(dB) on BSD68.}\label{tab:lessdata}
%     \begin{tabular}{lrcccc}
%         \toprule
%         \multirow{2}{*}{Method}      & \multirow{2}{*}{Params} & \multicolumn{4}{c}{Training images}                                                     \\
%                                      &                         & 400                                 & 200             & 100            & 50             \\ \midrule
%         % BM3D & - &  \multicolumn{4}{c}{31.07} \\
%         DnCNN \cite{zhang2017beyond} & 556k                    & 31.73                               & 31.65           & 31.47          & 31.23          \\ \midrule
%         TV \textit{extra-grad}       & 480                     & 30.75                               & 30.72           & 30.67          & 30.66          \\
%         Sparse coding                & 68k                     & 31.49                               & 31.49           & 31.46          & 31.40          \\
%         Group + Var                  & 68k                     & \textbf{31.75}                      & \textbf{31.66 } & \textbf{31.62} & \textbf{31.54} \\
%         \bottomrule
%     \end{tabular}
%     \vspace*{-0.5cm}

% \end{table}



==> A Flexible Framework for Designing Trainable Priors with Adaptive Smoothing and Game Encoding/impact.tex <==
Our main field of application is in image processing, with a focus on image
restoration and reconstruction, whose benefits for society are clear and well
established, even though a misuse of such a technology is of course possible;
for instance, the same total variation penalty may be used in medical imaging, for personal photography,
in astronomical imaging, or for restoring images produced by military devices.
More specifically, our paper is addressing the issue of interpretability of neural
networks, by considering models admitting a functional (mathematical) description of 
their decision functions, and with less parameters than classical deep learning models.
As we mentioned in the discussion section, we believe that these are first
steps to build systems producing explanable decisions, and that are more
data and energy efficient. These are important issues going beyond image processing,
which we would like to address in future work.



==> A Flexible Framework for Designing Trainable Priors with Adaptive Smoothing and Game Encoding/introduction.tex <==
Despite the undeniable successes of deep learning in domains as varied as
image processing~\cite{zhang2017beyond} and recognition~\cite{he2016deep},
 natural language processing~\cite{collobert2008unified}, speech~\cite{oord2016wavenet}
 or bioinformatics~\cite{alipanahi2015predicting},
feed-forward neural networks are often maligned as being ``black boxes''
that, except perhaps for their top classification or regression layers,
are difficult or even impossible to interpret.
In imaging applications, for example, the elementary operations typically 
consist of convolutions and pointwise nonlinearities, with many parameters
adjusted by backpropagation, and no obvious functional interpretation.
% For this reason, a recent line of research has focused on a posteriori interpretation;
% given a trained model, the goal is to understand and explain the model predictions in terms of input variables, regardless of the internal mechanisms of the deep network,
% see \cite{montavon2018methods} for more formal discussions on the topic.

In this paper, we consider instead network architectures explicitly derived from an optimization algorithm, and
thus interpretable from a functional point of view. The first instance of this approach we are aware of is LISTA~\cite{gregor2010learning},
which provides a fast approximation of sparse coding. %, see also~\cite{chen2018theoretical,liu2018alista}. 
Yet, we are not content to design an architecture that provides a fast approximation to a given
optimization problem, but we also want to learn a data representation pertinent for the corresponding task. 
This yields an unusual machine learning paradigm, where one learns the parameters of a parametric objective function used
to represent data, while designing an optimization algorithm to minimize it efficiently. % look at Roots paper

Even though interpretability is not always necessary to achieve good prediction, this point of view, sometimes called algorithm unrolling~\cite{fletcher2018plug,monga2019algorithm}, has proven
successful for solving inverse imaging problems, providing effective and parameter-efficient models.
This approach allows the use of
domain-specific priors within trainable deep models, leading to a large number of applications such as
%  blind  deblurring~\cite{li2020efficient},
  compressive imaging~\cite{sun2016deep,zhang2018ista}, demosaicking~\cite{lecouat2020fully},
denoising~\cite{lecouat2020fully,scetbon2019deep,simon2019rethinking}, and  super-resolution~\cite{wang2015deep}
% , for example.
.

However, existing approaches are often limited to simple image
priors such as sparsity induced by the $\ell_1$-norm~\cite{simon2019rethinking}, or
differentiable regularization functions~\cite{lefkimmiatis2018universal}, and a general algorithmic framework for combining complex, possibly non-smooth,
regularization functions is still missing.
Our paper addresses this issue and is able to leverage a large class of image
priors such as total variation~\cite{rudin1992nonlinear}, the $\ell_1$-norm, structured sparse
coding~\cite{mairal2009non}, or Laplacian regularization, where local optimization problems interact
with each others.
The interaction can be local among direct neighbors on an image grid, or non-local, capturing for instance
similarities between spatially distant image patches~\cite{buades2005non,dabov2009bm3d}.

% In this context, learning should be interpreted as learning the data representation encoded by the network parameters 
% and used in the optimizer encoded by the network architecture. 
%In this context, learned model parameters are used in the optimizer encoded by the network architecture.
In this context, we adopt a more general and flexible point of view than the standard convex optimization paradigm,
% In this context, learning should be interpreted as estimating the network parameters encoding the data representation
and consider formulations to represent data based on non-cooperative games~\cite{nikaido1955note}
potentially involving non-smooth terms, which are tackled by using the Moreau-Yosida regularization
technique~\cite{hiriart2013convex,yu2013better}. Unrolling the resulting optimization algorithm
results in a network architecture that can be trained end-to-end and capture any combination
of the domain-specific priors mentioned above. 
This approach includes and improves upon specific trainable 
sparse coding models based on the $\ell_1$-norm for example~\cite{simon2019rethinking,wang2015deep}. 
More importantly perhaps, it can be used to construct several
 interesting new image priors:
In particular, we show that a trainable variant of total variation and
its non-local variant based on
self similarities is competitive with the state of the art in imaging
tasks, despite using up to 50 times fewer parameters, with corresponding
gains in speed.
We demonstrate the effectivness and the flexibility
of our approach on several imaging tasks, namely denoising, compressed fMRI reconstruction,
and stereo matching.

\vs
\paragraph{Summary of our contributions.}
First, we provide a new framework for building trainable variants of a large class of
domain-specific image priors.
%  thanks to smoothing techniques and game encoding.
Second, we show that several of these priors match or even outperform existing techniques that use a
much larger number of parameters and training data.
Finally, we present a set of practical tricks to make optimization-driven layers easy to train.



==> A Flexible Framework for Designing Trainable Priors with Adaptive Smoothing and Game Encoding/macros.tex <==
\newcommand\vsp{\vspace*{-0.1cm}}
\newcommand\vs{\vspace*{-0.1cm}}
\newcommand\yb{\mathbf{y}}
\newcommand\ab{\mathbf{a}}
\newcommand\Yb{\mathbf{Y}}
\newcommand\Ncal{\mathcal{N}}
\newcommand\vb{\mathbf{v}}
\newcommand\xb{\mathbf{x}}
\newcommand\Xb{\mathbf{X}}
\newcommand\Hb{\mathbf{H}}
\newcommand\Db{\mathbf{D}}
\newcommand\Ab{\mathbf{A}}
\newcommand\Ub{\mathbf{U}}
\newcommand\Pb{\mathbf{P}}
\newcommand\Fb{\mathbf{F}}
\newcommand\Zb{\mathbf{Z}}
\newcommand\ub{\mathbf{u}}
\newcommand\wb{\mathbf{w}}
\newcommand\zb{\mathbf{z}}
\newcommand\Cb{\mathbf{C}}
\newcommand\Ib{\mathbf{I}}
\newcommand\Wb{\mathbf{W}}
\newcommand\Rb{\mathbf{R}}
\newcommand\Mb{\mathbf{M}}
\newcommand\Bb{\mathbf{B}}
\newcommand\db{\mathbf{d}}
\newcommand\bb{\mathbf{b}}
\newcommand\rb{\mathbf{r}}


\newcommand\ones{\mathbf{1}}
\newcommand\Real{\mathbb{R}}
%\newcommand\alphab{\boldsymbol{\alpha}}
\newcommand\alphab{\mathbf{z}}
\newcommand\betab{\boldsymbol{\beta}}
\newcommand\Lambdab{\boldsymbol{\Lambda}}
\newcommand\Thetab{\boldsymbol{\Theta}}
\newcommand\thetab{\boldsymbol{\theta}}
\newcommand\Sigmab{\boldsymbol{\Sigma}}
\newcommand\kappab{\boldsymbol{\kappa}}
\newcommand\lambdab{\boldsymbol{\lambda}}

\newcommand\Pcal{{\mathcal{P}}}

\newcommand{\norm}[1]{\lVert#1\rVert}
\usepackage{pifont}% h
\newcommand{\cmark}{\ding{51}}
\newcommand{\xmark}{\ding{55}}
\newcommand{\blue}{\textcolor{blue}}

\def\eg{\emph{e.g.}} 
\DeclareMathOperator{\EX}{\mathbb{E}}% expected value
\DeclareMathOperator*{\argmax}{arg\,max}
\DeclareMathOperator*{\argmin}{arg\,min}
\DeclareMathOperator{\prox}{\text{Prox}}
\DeclareMathOperator{\sign}{sign}
\DeclareMathOperator{\soft}{soft}
\DeclareMathOperator{\diag}{diag}
\DeclareMathOperator{\e}{e}



==> A Flexible Framework for Designing Trainable Priors with Adaptive Smoothing and Game Encoding/method.tex <==
\subsection{Proposed Approach}

\vs
\begin{minipage}[]{.50\textwidth}
	We adopt a more general point of view than~(\ref{eq:bilevel}),
	where we assume that input signals admit a local ``patch'' structure (\eg, rectangular image regions) and the data
	representation encodes individual patches.
	Assuming that there are $m$ patches in~$\xb$, we denote by $\Zb^\star(\xb)=[\zb_{1}^\star(\xb), \ldots, \zb_{m}^\star(\xb) ]$ in $\Real^{p \times m}$
	the representation of~$\xb$ and by $\zb_j^\star(\xb)$ the representation of patch~$j$ (we omit the dependency on the model parameters~$\thetab$ for simplicity).
	In imaging applications and as in previous models~\cite{simon2019rethinking},  $\Zb^\star(\xb)$ can be seen as a feature map akin to that of a convolutional neural network with $p$ channels.
\end{minipage}%
\hspace{0.5cm}
\begin{minipage}[]{.43\textwidth}
	\centering
	\includegraphics[width=\textwidth]{diagram_layer.pdf}
	\captionof{figure}[b]{Our models encode locally an input feature vector. The local optimal solutions $\zb_j^\star$ interact trough the regularization function $\psi_\theta^j(\Zb)$.}\label{fig:diagram}
\end{minipage}
%
%\begin{figure}
%\centering
%   \captionof{figure}[b]{Illustration our feature encoding layer.}\label{fig:diagram}
%  \includegraphics[width=6.2cm]{diagram.pdf}
%\end{figure}

%We adopt a more general point of view than~(\ref{eq:bilevel}),
%where we assume that input signals admit a local ``patch'' structure (\eg, rectangular image regions) and the data
%representation encodes individual patches.
%Assuming that there are $m$ patches in~$\xb$, we denote by $\Zb^\star(\xb)=[\zb_{1}^\star(\xb), \ldots, \zb_{m}^\star(\xb) ]$ in $\Real^{p \times m}$
%the representation of~$\xb$ and by $\zb_j^\star(\xb)$ the representation of patch~$j$ (we omit the dependency on the model parameters~$\thetab$ for simplicity).
%In imaging applications and as in previous models~\cite{simon2019rethinking},  $\Zb^\star(\xb)$ can be seen as a feature map akin to that of a convolutional neural network with $p$ channels.



\vs
\paragraph{Encoding with non-cooperative convex games.}
Concretely, given a signal $\xb$, we denote by $\Pb_j \xb$ the
patch of $\xb$ centered at position~$j$, where $\Pb_j$ is a linear patch extraction operator,
and we define the optimal encoding $\Zb^\star(\xb)$ of $\xb$ as a Nash equilibrium of the set of problems
\begin{equation}
	\min_{\alphab_j \in {\mathcal Z}} h_{\thetab}(\Pb_j \xb,\alphab_j) + \psi_{\thetab}^j(\Zb)~~~~\text{for}~~j=1,\ldots,m, \label{eq:formulation}
\end{equation}
where $h_{\thetab}$ is a a convex reconstruction objective for each patch,
parametrized by $\thetab$, $\psi_{\thetab}^j$ is a convex regularization function
encoding interactions between the
variable $\zb_j$ and the remaining ones $\zb_l$ for $l\neq j$, and $\mathcal Z$ is a convex subset of $\Real^p$.
When $\mathcal Z$ is compact, the problem is a specific instance of
a non-cooperative convex game~\cite{nikaido1955note}, which is known
to admit at least one Nash equilibrium---that is, a solution such that one of the objectives in~(\ref{eq:formulation})
is optimal with respect to its variable~$\zb_j$ when the other
variables~$\zb_{l}$ for $l\neq j$ are fixed. The conditions under which an
optimization algorithm is guaranteed to return such an equilibrium point
are well studied, see Section~\ref{sec:optim}, and in many situations the compactness
of $\mathcal Z$ is not required, as also observed in our experiments where we choose $\mathcal Z = \Real^p$.
For instance, in several practical cases,
(\ref{eq:formulation}) can be solved by minimizing the sum
of~$m$ convex terms, a setting called a \emph{potential game}, which boils
down to a classical convex optimization problem.
% \textcolor{red}{highlight difference games vs bilevel \ref{eq:bilevel}  more explicitely cf R2}

\subsection{Application of our Framework to Inverse Imaging Problems}
	
\vs
In this section, we show how to leverage our optimization-driven layers for imaging. For the sake of clarity we choose to narrow down the scope of this presentation to imaging, even though our method is not limited to this single application: different modalities including for example genomic/graph data could benefit from our methodology. 

% While our approach is generic and hence not limited to imaging problems, we choose to limit our presentation to imaging applications. Our approach is appealing for solving imaging problems, as it allows the use of classical image priors within deep models that are trainable end-to-end.

\vsp
\paragraph{Examples of models $h_{\thetab}$.}
We consider two cases in the rest of this presentation:
\begin{itemize}[leftmargin=*,nosep]
      \item \emph{Pixel reconstruction}: $h_{\thetab}(\Pb_j \xb, \zb_j) = (\xb_j - \zb_j)^2$, where $\xb_j$ is the pixel~$j$ of $\xb$
       and $\zb_j$ is a scalar, corresponding to patches of size $q=1 \times 1$ and $p=1$.
      \item \emph{Patch encoding on a dictionary}: $h_{\thetab}(\Pb_j \xb, \zb_j) = \|\Pb_j \xb_j - \Db \zb_j\|^2$, where $\Db$ in $\Real^{q \times p}$ is a dictionary,~$q$ is the patch size, and $p$ is the number of dictionary elements. This is a classical model where patch $j$ is approximated by a linear, often sparse, combination of dictionary elements~\cite{elad2006image}.  
\end{itemize}
Only the second choice involves model parameters $\Db$ (represented by $\thetab$). These
two loss functions are common in  image
processing~\cite{elad2006image}, but other losses may be used for other modalities.

\vsp
\paragraph{Linear reconstruction with a dictionary.}

Assuming that $\yb$ and $\xb$ have the same size~$m$ for simplicity, predicting $\yb$ from a feature map $\Zb^\star(\xb)$
is typically achieved by using a learned dictionary matrix $\Wb$ in $\Real^{q \times p}$ where $q$ is the patch size.
Then, $\Wb \zb_j^\star(\xb)$\footnote{We employ a debiasing dictionary $\Wb \neq \Db$ to improve the quality of the reconstructions. Debiaising is commonly used when dealing with $\ell_1$ penalty which is known to shrink the coefficients $\Zb$ too much.} can be interpreted as a reconstruction of the $j$-patch
of~$\yb$ .
Since the patches overlap, we obtain $q$ estimators for every pixel,
which can be combined by averaging (neglecting border effects below for simplicity), yielding the prediction
\begin{equation}
	\hat{\yb}(\xb,\theta, \Wb) = \frac{1}{q} \sum_{j=1}^m \Pb_j^\top \Wb \zb^\star_j(\xb), \label{eq:averaging}
\end{equation}
where $\Pb_j^\top$ is the linear operator that places a patch of size $q$ at position $j$ in a signal of dimension~$m$.
Patch averaging is a classical operation in patch-based image restoration algorithms, see~\cite{elad2006image},
which can be interpreted in terms of transposed convolution\footnote{\texttt{torch.nn.functionnal.conv2D\_transpose} on PyTorch~\cite{pytorch}.
} and admits fast implementations on GPUs. 
% See Figure \ref{fig:diagram2} for a schematic representation of the models architecture for image restoration.

\vs
\paragraph{Learning problem.} For image restoration,
 given training pairs of corrupted/clean images $\{\xb_i,\yb_i\}_{i=1,\ldots,n}$, we consider the regression problem
$	\min_{ \thetab \in \Theta, \Wb \in \Real^{q \times p}} \| \yb_i - \hat{\yb}(\xb_i,\theta, \Wb)\|^2~~~~\text{where}~~\hat{\yb}(\xb_i)
  ~~\text{is defined in~(\ref{eq:averaging})}$. 
  

\begin{figure}[t]
	\centering
\includegraphics[width=0.80\textwidth]{diagram_model.pdf}
\captionof{figure}[b]{Architecture of our trainable models for image restoration.}\label{fig:diagram2}
\vspace{-0.4cm}
\end{figure} 

% \vs
% For patch-based models we employ a debiasing dictionary $\Wb$ to improve the quality of the reconstructions.
% Debiaising is commonly used when dealing with $\ell_1$ penalty which is known to shrink the coefficients $\Zb$ too much. 
% In our method, $\Wb$ is learned through backpropagation (you can refer to the Algorithm \ref{alg:pseudo} below).
% However, when dealing with pixel-based regularizers (including TV) we are in the setup where $q = 1 \times 1 \text{ and } p = 1$: the $\Wb$ matrix boils down to a single scalar coefficient
% that can be neglected for the sake of a simpler implementation. 

\input{priors}

\begin{algorithm}[]

  \caption{Pseudocode of the general training procedure for image restoration}\label{alg:pseudo}
  \begin{algorithmic}[1]
      \State Sample a minibatch of pairs of corrupted/clean images $\{(\xb_0,\yb_0), \cdots, (\xb_K,\yb_K)\}$;
      \State Extract overlapping patches of corrupted images to form tensors $\mathbf{X}_i=[\Pb_1 \xb_i , \cdots, \Pb_n \xb_i]$;
      \For {$t=1,2,\ldots,K$} \Comment{Compute an approximate Nash equilibrium $\Zb^\star$ of the convex games}
      \State $\Zb_{t+1} \leftarrow \Zb_{t} -\eta_t H_\theta(\Zb_{t},\Xb)$;
      \EndFor 
      \State Approximate clean images by linear reconstruction $\hat{\yb}  = \frac{1}{q} \sum_{j=1}^m \Pb_j^\top \Wb
          \zb^\star_{j}(\Xb,\theta)$;
      \State Compute the $\ell_2$ reconstruction loss $ \|\yb - \hat{\yb}(\xb,\theta,\Wb) \|_2^2$ on the minibatch;
      \State Compute an estimate of the gradients wrt.  $(\theta, \Wb)$ with auto-diff;
      \State Update trainable parameters $(\theta, \Wb)$ with Adam;
      % \Function{<name>}{<params>} <body> \EndFunction
  \end{algorithmic}
%   \vspace{-0.4cm}
\end{algorithm}

\vspace{-0.2cm}
\subsection{Differentiability and End-to-end Training}\label{sec:optim}

In this section we adress end-to-end training of the optimization-driven layers.
% Given training pairs of corrupted/clean data $\{\xb_i,\yb_i\}_{i=1,\ldots,n}$, we consider the learning problem
% \begin{equation}
% 	\min_{ \thetab \in \Theta, \Wb \in \Real^{q \times p}} \| \yb_i - \hat{\yb}_{\theta, \Wb}(\xb_i)\|^2~~~~\text{where}~~\hat{\yb}(\xb_i)
% 	~~\text{is defined in~(\ref{eq:averaging})}, \label{eq:loss} 
% \end{equation}
Given pairs of training data $\{\xb_i,\yb_i\}_{i=1,\ldots,n}$, we consider the learning problem
\begin{equation} \label{eq:learning}
  \min_{\thetab \in {\Theta}}   
  \frac{1}{n}\sum_{i=1}^n L \left( \yb_i, g_\theta \left (\alphab^\star_{\thetab}(\xb_i) \right ) \right),
 % \left [ f_S(\hat{x}_S^*(\theta) , \theta) \right ] \quad
 %  \text{s.t.} \quad  \hat{x}_S^*(\theta) \approx \argmin_{x} h_S(x,\theta) ,
 % why linear WZ ? looks very specific
\end{equation}
% and 
where $g_\theta$ is a differentiable function. We consider the approximation where the codes~$\zb_j^\star(\xb)$ are
obtained as the $K$-th step of an optimization algorithm for solving the
problem~(\ref{eq:formulation}). To obtain these codes,
we leverage (i) iterative gradient and extra-gradient methods, which are classical
for solving game problems~\cite{bertsekas1989parallel,facchinei2007finite},
and (ii) a smoothing technique for dealing with the regularization functions~$\psi_{\thetab}^j$ above when they are non-smooth.
Refer to Algorithm \ref{alg:pseudo} for an overview of the training procedure.
We start with the first point when dealing with smooth objectives.

\vs
\paragraph{Unrolled optimization for convex games.}
Consider a set of~$m$ objective functions of the form
\begin{equation}
	\min_{\zb_j \in \Real^p} h_j(\Zb) ~~~~\text{with}~~~~\Zb=[\zb_1,\ldots,\zb_m],\label{eq:convexgame}
\end{equation}
where the functions $h_j$ are convex and differentiable and may depend on other parameters
than~$\zb_j$. 
% =============
Our objective is to find a zero of the simultaneous gradient
% We begin by looking at techniques that were developed  to solve variational
% inequalities~\cite{bertsekas1989parallel,facchinei2007finite,juditsky2011solving,mertikopoulos2018optimistic},
% which, for the problem we consider, are designed for finding a zero of the simultaneous gradient
\begin{equation}
	H(\Zb) = [\nabla_{\zb_1} h_1(\Zb) ,  \cdots , \nabla_{\zb_m} h_m(\Zb)  ],
\end{equation}
which corresponds to a Nash equilibrium of the game~(\ref{eq:convexgame}).
In the rest of this presentation,
we consider  both the general setting and the simpler case of 
so-called potential games, for which the equilibrium can be found as the optimum of a single convex objective.
% In our paper, we consider
% such a general case, but we remark that some of our regularization functions lead to a so-called
% potential game, which is equivalent to minimizing a single convex objective. 
This is the case for several of our regularizers, for example the TV penalty with symmetric weights. More details are provided in
Appendix~\ref{appendix:potential} on the nature of the non-cooperative games corresponding to our penalties.

Two standard methods studied in the variational inequality litterature~\cite{bertsekas1989parallel,facchinei2007finite,juditsky2011solving,mertikopoulos2018optimistic} 
are the \textit{gradient} and the \textit{extra-gradient}~\cite{korpelevich1976extragradient} methods.
The iterates of the basic gradient method are given by
\begin{equation}
	\Zb_{t+1} = \Zb_{t} - \eta_t H(\Zb_t), \label{eq:gd}
\end{equation}
where $\eta_t > 0$ is a step-size. These iterates are known to converge under a
condition called strong monotonicity of the operator~$H$, which is related to the concept
of strong convexity in optimization, see~\cite{bertsekas1989parallel}. Because
this condition is relatively stringent, the extra-gradient method is often
prefered~\cite{korpelevich1976extragradient}, as
it is known to converge under weaker conditions, see~\cite{juditsky2011solving,mertikopoulos2018optimistic}.
The intuition of the method is to compute a look ahead step in order to compute more stable directions of descent:
\begin{equation}
	\begin{split}
		\text{Extrapolation step} \quad & \Zb_{t+1/2} = \Zb_{t} - \eta_t H(\Zb_t)       \\
		\text{Update step} \quad        & \Zb_{t+1} = \Zb_{t} - \eta_t H(\Zb_{t+1/2}).
	\end{split}\label{eq:extragd}
\end{equation}
In this paper, our strategy is to unroll iterates of one of these two algorithms, and then
to use auto differentiation for  learning the model parameters~$\thetab$.
% In this paper, our strategy is to unroll iterates of one of these two algorithms, allowing
% us to use auto differentiation for computing the gradient learning the model parameters~$\thetab$.
%
Furthermore, parameters that control the optimization process (\eg, step size
$\eta_t$) can also be learnt with this approach.
%
It should be noted that optimization-driven layers have never been
used before in the context of non-cooperative games, to the best of our knowledge, and therefore an empirical study is
needed to choose between the strategies~(\ref{eq:gd}) or~(\ref{eq:extragd}).
In our experiments,
extra-gradient descent has always performed at least as well, and
sometimes significantly better, than plain gradient descent for
comparable computational budgets.
See for example Table~\ref{table:expgd} for a smoothed variant of the TV penalty.
\begin{table}[]
	\caption{Gradient descent (GD) vs. Extra-gradient. Denoising results in avg. PSNR with $\sigma=25$ on BSD68~\cite{martin2001database}.}\label{table:expgd}
	\centering
	\begin{tabular}{lccc}
		\toprule
		{Method}                         & GD (24 iters) & GD (48 iters) & Extra-gradient (24 iters) \\
		\midrule
		Trainable TV \textit{symmetric}  & 27.58         & 27.50         & 27.82                     \\
		Trainable TV \textit{assymetric} & 27.99         & 27.89         & 28.24                     \\
		\bottomrule
	\end{tabular}
\end{table}

\paragraph{Moreau-Yosida smoothing.} 
The non-smooth regularization functions we consider can be written as a sum of simple terms. 
Omitting the dependency on $\thetab$ for simplicity, we may indeed write
\begin{displaymath}
	\psi^j(\Zb) =  \textstyle \sum_{k=1}^r  \phi_k( L_{k,j}(\Zb))~~~~\text{for some}~r \geq 1,
\end{displaymath}
where $L_{k,j}$ is a linear mapping and $\phi_k$ is either the $\ell_1$- or $\ell_2$-norm. For
instance, $\phi_k$ is the $\ell_1$-norm with $L_{k,j}(\Zb) = a_{k,j}(\zb_j -\zb_k)$ in $\Real^p$ for the TV
penalty, and $L_{k,j}(\Zb) = [ \sqrt{a_{1,j}}\zb_1(k), \ldots, \sqrt{a_{1,j}}\zb_q(k)]^\top$ in $\Real^q$ with
$\phi_k$ being the $\ell_2$-norm for the non-local group regularization. 
% where $L_{k,j}$ is a linear mapping and $\phi_k$ is either the $\ell_1$- or $\ell_2$-norm. For
% instance, $\phi_k=\ell_1$ with $L_{k,j}(\Zb) = a_{k,j}(\zb_j -\zb_k)$ in $\Real^p$ for the TV
% penalty, and $L_{k,j}(\Zb) = [ \sqrt{a_{1,j}}\zb_1(k), \ldots, \sqrt{a_{1,j}}\zb_q(k)]^\top$ in $\Real^q$ with
% $\phi_k=\ell_2$ for the non-local group regularization. 
Handling such non-smooth convex terms
may be achieved by leveraging the so-called Moreau-Yosida
regularization~\cite{lemarechal1997practical,moreau1962fonctions,yosida}
\begin{displaymath}
	\Phi_k(\ub) =   \min_{\vb} \left\{\phi_k(\vb) + \frac{\alpha}{2}\|\vb - \ub\|^2\right\},
\end{displaymath}
which defines an optimization problem whose solution is called the proximal
operator~$\text{Prox}_{\phi_k/\alpha}[\ub]$. As shown in~\cite{lemarechal1997practical}, $\Phi_k$ is
always differentiable and $\nabla \Phi_k(\ub) = \alpha(\ub - \text{Prox}_{\phi_k/\alpha}[\ub])$,
which can be computed in closed form when $\phi_k=\ell_1$ or~$\ell_2$. The positive parameter $\alpha$
controls the trade-off between smoothness (the gradient of $\Phi_k$ is $\alpha$-Lipschitz) and the
quality of approximation. It is thus natural to define a smoothed approximation~$\Psi^j$ of
$\psi^j$ as $\Psi^j(\Zb)  =  \sum_{k=1}^r  \Phi_k( L_{k,j}(\Zb))$.

Note that when the proximal operator of $\psi^j$ can be computed efficiently, as is the case for the
$\ell_1$-norm, gradient descent algorithms can typically be adapted to handle the non-smooth
penalty without extra computational cost~\cite{mairal2014sparse}, and there is no need for
Moreau-Yosida smoothing. However, the proximal operator of the TV penalty and the non-local group
regularization do not admit fast implementations.  For the first one, computing the proximal operator
requires solving a network flow problem~\cite{chambolle2009total}, whereas the second one is
essentially easy to solve when the weights $a_{j,k}$ form non-overlapping groups of variables,
leading to a penalty called group Lasso~\cite{turlach}.

We are now ready to present our unrolled algorithm as we have previously discussed
gradient-based algorithms for solving convex smooth games and a smoothing
technique for handling non-smooth terms.
Generally, at iteration~$t$, the gradient algorithm~(\ref{eq:gd}) performs the following simultaneous updates for all problems~$j$
\begin{displaymath}
	\begin{split}
		\ub_{k,j}^{(t)}~~~  &\leftarrow \prox_{\phi_k/\alpha_{k,t}}[L_{k,j} (\Zb^{(t)})]~~~~~~\text{for}~~k=1,\ldots,r                                     \\
		\zb_j^{(t+1)} &\leftarrow \zb_j^{(t)} - \eta_t \left ( \nabla_{\zb_j} h_\theta\left(\Pb_j \xb,\zb_j^{(t)}\right) + \sum_{k=1}^r \alpha_{k,t} \: \left[L_{k,j}^* \left  (L_{k,j}(\Zb^{(t)})- \ub_{k,j}^{(t)} \right ) \right]_j\right ),\\
	\end{split}
\end{displaymath}
where $L_{k,j}^*$ is the adjoint of the linear mapping $L_{k,j}$. 
The computation of the gradients can be implemented with simple operations
allowing auto-differentiation in deep learning frameworks.
Interestingly, the smoothing parameter $\alpha$ can be made iteration-dependent, and learned
along with other model parameters such that the amount of smoothing is chosen automatically.  


\subsection{Tricks of the Trade for Unrolled Optimization}\label{sec:tricks}

Our strategy is to unroll iterates of our algorithms, and then
% compute gradient of the model parameters ~$\thetab$ with respect to the reconstruction loss by leveraging auto-differentiation for learning the model parameters.
compute  $\nabla_{\thetab} \zb_{\thetab}^\star$ by automatic differentiation.
% use auto differentiation for learning the model parameters~$\thetab$.
%
We present here a set of practical rules, some old and some new, facilitating 
training when $h_{\thetab}$ is a patch encoding function on a dictionary~$\Db$.
\vsp
\paragraph{Initialization.}
To help the algorithm converge, we choose an initial stepsize~$\eta_t \leq \frac{1}{L}$,
where $L$ is the Lipschitz constant of $\nabla_{\zb} h_{\thetab}$, which
is the classical step-size used by ISTA~\cite{beck2009fast}. To do so, inspired by
\cite{simon2019rethinking} we normalize the initial dictionary by its largest singular value and 
take $\eta_0=1$.
Note that we can go one step further and normalize the dictionary throughout the training phase.
This is in fact equivalent to the spectral normalization that has received some attention
recently, notably for generative adversarial networks \cite{miyato2018spectral}.

\vs
\paragraph{Untied parameters.}
In our framework, $ \nabla_{\zb_j} h_{\thetab}(\Pb_j \xb, \zb_j)=\Db^\top \left ( \Db \zb_j
- \Pb_j \xb \right) $. It has been suggested in previous
work~\cite{gregor2010learning,lecouat2020fully,simon2019rethinking} to introduce an additional 
parameter~$\Cb$ of the same size as~$\Db$, and consider instead the parametrization $ \Cb^\top
\left ( \Db \zb_j - \Pb_j \xb \right) $, $\Cb$ acting as a learned preconditioner. Even though the theoretical effect of this modification is not fully
understood, it has been observed to accelerate convergence and boost performance for denoising tasks~\cite{lecouat2020fully}. In our experiments, we will indicate in
which cases we use this heuristic.

\vs
\subparagraph{Backtracking.}
A simple way for handling the potential instability of the unrolled algorithm is to use a
backtracking scheme which automatically decreases the stepsize when
the training loss diverges. This heuristic was used for instance in  \cite{lecouat2020fully}. 
More details are provided in Appendix~\ref{appendix:training}.


\vsp
\subparagraph{Barzilai-Borwein method for choosing the stepsize.}
A different, perhaps more principled, approach to improved stability consists in adaptively
choosing an adaptive stepsize $\eta_t$. The
literature on convex optimization proposes a set of effective rules,
known as Barzilai-Borwein (BB) step size rules~\cite{wright2009sparse}. Even though these rules were not
designed for convex games, they appear to be very effective in practice in the context of our
optimization-driven layers. Concretely, they lead to
step sizes $\eta_{t,j} = { \| \Db^\top \Db \mathbf{s}_j \|_2}/{ \| \Db \mathbf{s}_j \|^2}$ with
${\mathbf s}_j = \zb_j^{(t)}- \zb_j^{(t-1)}$ for problem~$j$ at iteration~$t$.


%\begin{minipage}[t]{.54\textwidth}
%In our experiments, we observed that spectral normalization, backtracking, and Barzilai-Borwein step size were all effective to stabilize
%training. We have noticed that the spectral normalization impacts negatively the reconstruction accuracy,
%while the BB method tend to improve it by using larger stepsizes, at the
%expense of a larger computational cost. This is illustrated in Table \ref{tab:stability} for a
%smoothed variant of sparse coding (we indicate with a crossmark when the algorithm diverges). In addition, we observe that the untied models brings a small
%boost in reconstruction accuracy. \end{minipage}% 
%\hspace{0.2cm}
%\begin{minipage}[t]{.45\textwidth}
%  \centering
%  \vspace{-0.2cm}
%  \captionof{table}{Study of stabilization techniques for learnt sparse coding. Denoising results in PSNR with $\sigma = 25$ on BSD68.}\label{tab:stability}
% {
%  \small
%  \begin{tabular}{lcccc}
%    \toprule
%    \multirow{2}{*}{Method}            & \multicolumn{2}{c}{Psnr (dB)}
%    \\
%
%                                             & D & C,D \\
%    \midrule
%    BM3D \cite{dabov2007image} & \multicolumn{2}{c}{28.57} \\
%
%    Sparse Coding (SC)                    & \xmark   & \xmark  \\ 
%     SC + Backtracking & 28.71                         & 28.83                                   \\
%     SC + Spectral norm & 28.69                         & 28.82                                   \\
%     SC + Barzilai-Borwein & 28.82                         & \textbf{28.86}
%                                        \\ % experimenting || DtDs || / || Ds|| 
%    \bottomrule
%  \end{tabular}
%
%  } 
%\end{minipage}
\vspace{0.25cm}
\begin{minipage}[]{.42\textwidth}
	\centering
	\vspace{-0.25cm}
	\captionof{table}{Study of stabilization techniques for learnt sparse coding. Denoising results in average PSNR with $\sigma = 25$ on BSD68.}\label{tab:stability}
	{
		\small
		\begin{tabular}{lcccc}
			\toprule
			\multirow{2}{*}{Method}            & \multicolumn{2}{c}{Psnr (dB)}
			\\
			
			                      & D      & C,D            \\
			\midrule
			BM3D \cite{dabov2007image} & \multicolumn{2}{c}{28.57} \\
			
			Sparse Coding (SC)    & \xmark & \xmark         \\ 
			SC + Backtracking     & 28.71  & 28.83          \\
			SC + Spectral norm    & 28.69  & 28.82          \\
			SC + Barzilai-Borwein & 28.82  & \textbf{28.86} 
			\\ % experimenting || DtDs || / || Ds|| 
			\bottomrule
		\end{tabular}
		
	} 
\end{minipage}
\hspace{0.2cm}
\begin{minipage}[]{.532\textwidth}
	In our experiments, we observed that spectral normalization, backtracking, and Barzilai-Borwein step size were all effective to stabilize
	training. We have noticed that the spectral normalization impacts negatively the reconstruction accuracy,
	while the BB method tend to improve it by using larger stepsizes, at the
	expense of a larger computational cost. This is illustrated in Table \ref{tab:stability} for a
	smoothed variant of sparse coding (we indicate with a crossmark when the algorithm diverges). In addition, we observe that the untied models brings a small
	boost in reconstruction accuracy. \end{minipage}% 
	
	% \footnotetext{Crossmarks indicates when the algorithm did not converge.}
	
	\vsp
	
	 
	 


==> A Flexible Framework for Designing Trainable Priors with Adaptive Smoothing and Game Encoding/priors.tex <==
% We will show how our framework can be used t
%We will now present several instances of formulations~(\ref{eq:formulation}).


\vs
\paragraph{Examples of regularization functions $\psi_{\thetab}^j$.} Our framework allows the use of several regularization 
functions, which are presented
in the table \ref{table:priors} below. 
We assume that the patches are nodes in a graph, and denote by~${\mathcal N}_j$ the set of neighbors of the patch $j$.
For natural images, the graph may be a two-dimensional grid with edge weights~$a_{j,k}$ that depend on the relative position of the patches~$j$ and~$k$, which we denote by $a_{j\text{--}k}$, 
but it may also be a non-local graph based on some similarity function as in~\cite{lecouat2020fully,liu2018non}. 
Concretely, we can consider:
\begin{itemize}[leftmargin=*,nosep]
\item the distance $d^{j,k}_\mathrm{NL} = \| \diag(\kappab) ( \Pb_j \xb - \Pb_k \xb )\|^2$
between patches~$j$ and $k$ of the image~$\xb$,
 where $\kappab$ in $\Real^q$ is a set of parameters to learn, and $q$ is the patch size,
and we define normalized weights $ a_\mathrm{NL}^{j,k} = {e^{-d^{j,k}_\mathrm{NL} }}/{\sum_{l \in \mathcal{N}_j} e^{-d^{j,k}_\mathrm{NL} }}$.
%\item or a distance inspired from the bilateral filter \cite{tomasi1998bilateral}. In that case we define the normalized weights $$ a_\mathrm{BL}^{j,k} = {e^{-\| \xb_i - \xb_j \|_2^2/\sigma_i}e^{-\|i - j \|_2^2/\sigma_r}}/{\sum_{l \in \mathcal{N}_j} \left ( {e^{-\| \xb_i - \xb_j \|_2^2/\sigma_i}e^{-\|i - j \|_2^2/\sigma_r}} \right ) }.$$
\item or a distance inspired from the bilateral filter \cite{tomasi1998bilateral}. In that case we define the distance  $d^{j,k}_\mathrm{BL} = \frac{\| \xb_i - \xb_j \|^2}{2\sigma_d^2}+ \frac{\|i - j \|^2}{2\sigma_r^2}$ between pixels on a local window  $ \mathcal{N}_j $ centered around pixel $j$, and we define again normalized weights $ a_\mathrm{BL}^{j,k} = {e^{-d^{j,k}_\mathrm{BL}}}/{\sum_{l \in \mathcal{N}_j} e^{-d^{j,k}_\mathrm{BL}}}$.
\end{itemize}


%\textcolor{red}{Talk about bilateral here}

 

% \begin{itemize}[leftmargin=*,nosep]
%    \item \emph{Total variation (TV) and its graph variant}: Assume that for each pair of patches $(j,l)$, there is a weight~$a_{j,l}$ encoding the influence of patch $l$ over patch $j$. Then, it is easy to define matrices~$\Ab_j$ such that     
%       $\psi(\Zb \Ab_j) = \sum_{l=1}^j a_{j,l}\| \zb_j - \zb_l\|_1$. Such a penalty may be used when the weights encode symmetric relations---that is $a_{j,l}=a_{l,j}$. In such a case, our setting recovers the total variation penalty on a graph (which may be a grid for images). Our setup is however not limited to symmetric relations, which, to the best of our knowledge, has never been considered before.
%    \item \emph{Laplacian regularization}: We consider the same setup as the previous total variation penalty, but we define $\psi(\Zb \Ab_j) = \sum_{l=1}^j a_{j,l}\| \zb_j - \zb_l\|^2$. 
%    \item \emph{Sparse coding and the $\ell_1$-norm}: We may also consider the simple setup when $\psi(\Zb\Ab_j) = \|\zb_j\|_1$, which yields independent optimization problems.
%    \item \emph{Structured sparse coding on graphs}: 
%    \item \emph{Variance reduction}:
% \end{itemize}
%Should add REFS
%example of useful graph: non-local
%should do a table, would be nicer

%\begin{table}
   %\caption{Examples of regularization functions $\psi_{\thetab}$}  
         \captionof{table}[t]{A non-exhaustive list of regularization functions $\psi_{\thetab}$ covered by our framework.}\label{table:priors}
   \begin{center}
   \renewcommand{\arraystretch}{1.5}
   \begin{tabular}{|c|c|c|c|c|}
      \hline
      & $\psi_{\thetab}^j(\Zb)$  & Model parameters \\ 

      \hline
      Laplacian & $\sum_{k \in {\mathcal N}_j} a_{j\text{--}k}\| \zb_j - \zb_k\|^2$ & weights in $\Real^{|{\mathcal N}|}$ \\    
      \hline
      Non-local Laplacian & $\sum_{k \in {\mathcal N}_j} a_\mathrm{NL}^{j,k}\| \zb_j - \zb_k\|^2$ & $\kappab$ in $\Real^q$ \\    
       \hline
      Bilateral filter (BF) & $\sum_{k \in {\mathcal N}_j} a_\mathrm{BL}^{j,k}\| \zb_j - \zb_k\|^2$ &  $\sigma_d \in \Real$ and $\sigma_r \in \Real$  \\    
      \hline
      Total variation (TV) & $\sum_{k \in {\mathcal N}_j} a_{j\text{--}k}\| \zb_j - \zb_k\|_1$ &  weights in $\Real^{|{\mathcal N}|}$  \\    
      \hline
      Non-local total variation (NLTV) & $\sum_{k \in {\mathcal N}_j}  a_\mathrm{NL}^{j,k}\| \zb_j - \zb_k\|_1$ & $\kappab$ in $\Real^q$\\          
            \hline
      Bilateral TV (BLTV) & $\sum_{k \in {\mathcal N}_j} a_\mathrm{BL}^{j,k}\| \zb_j - \zb_k\|_1$ & $\sigma_d \in \Real$ and $\sigma_r \in \Real$  \\   
      \hline
      Weighted $\ell_1$-norm (sparse coding)& $\sum_{l=1}^p \lambda_{l}|\zb_j[l] |$ & $\lambdab$ in $\Real^{p}$   \\    
      \hline
      Non-local group regularization & $\sum_{l=1}^p \lambda_l \sqrt{\sum_{k \in {\mathcal N}_j}a_{j,k}\zb_k[l]^2}$ & $\lambdab$ in $\Real^p$ and $\kappab$ in $\Real^q$ \\ 
      \hline
      Variance reduction &  $ \|\Wb \zb_j - \Pb_j \hat{\yb} \|^2$ with $\hat{\yb}$ from (\ref{eq:averaging}) &  $\Wb$ from~(\ref{eq:averaging}) \\ 
      \hline
   \end{tabular}
   \end{center}

%\end{table}

\paragraph{Novelty of the proposed formulation and relation to previous work.}
\begin{itemize}[leftmargin=*,nosep]
   \item \emph{Total variation}: to the best of our knowledge, the basic anisotropic TV
      penalty~\cite{chambolle2010introduction} does not seem to appear in the literature  on
      unrolled algorithms with end-to-end training. Note also that our TV variant allows
      learning non-symmetric weights $a_{j,k} \neq a_{k,j}$, leading to a
      non-cooperative game that goes beyond the
      classical convex optimization framework typically used with the TV penalty.
   \item \emph{Non-local TV}: the non-local TV penalty
      presented above is based on a classical formulation~\cite{gilboa2009nonlocal}, but can be incorporated 
      within a trainable deep
      network with non-symmetric weights.  
   \item \emph{Bilateral filtering}: the bilateral filter and its TV variant implemented in this paper are based on classical formulations \cite{tomasi1998bilateral,farsiu2004advances}. But they have not, to the best of our knowledge, been implemented as trainable priors.
   \item \emph{Sparse coding and variance reduction}: the weighted $\ell_1$-norm combined with the patch encoding
    loss~$h_{\thetab}$ yields a sparse coding formulation (SC) that has been well studied within optimization-driven 
    layers~\cite{scetbon2019deep,simon2019rethinking}. Yet, the  codes~$\zb_j$ in the SC setup are obtained by solving
     independent optimization problems, which has motivated by Simon and Elad~\cite{simon2019rethinking} to propose instead a 
     Convolutional Sparse Coding model (CSC),     
       where the full image is approximated by a linear combination of small
       dictionary elements.
       Unfortunately, as noted in~\cite{simon2019rethinking}, CSC leads to ill-conditioned optimization problems,
        making a hybrid approach between SC and CSC more effective. Our paper proposes an alternative solution 
        combining the weighted $\ell_1$-norm regularization  with a variance reduction penalty, 
        which forces the codes $\zb_j$ to reach a consensus when reconstructing the image~$\hat{\yb}$. 
        Our experiments show that this approach outperforms~\cite{simon2019rethinking} for image denoising.
    \item \emph{Non-local group regularization}: This 
       regularization function corresponds to a soft variant of the Group Lasso
       penalty~\cite{turlach}, which encourages similar patches to share
       similar sparsity patterns (set of non-zero elements of the
       codes~$\zb_j$). It was originally used in~\cite{mairal2009non} and was recently revisited within optimization-driven layers with an heuristic algorithm~\cite{lecouat2020fully}.
       Our paper provides a better justified algorithmic framework as well as the ability to combine  this penalty with other ones. 
\end{itemize}

